Unveiling A Hidden Risk: Exposing Educational but Malicious Repositories in GitHub

Are malicious repositories hiding under the educational label in GitHub? Recent studies have identified collections of GitHub repositories hosting malware source code with notable collaboration among the developers. Thus, analyzing GitHub repositories deserves inevitable attention due to its open-source nature providing easy access to malicious software code and artifacts. Here we leverage the capabilities of ChatGPT in a qualitative study to annotate an educational GitHub repository based on maliciousness of its metadata contents. Our contribution is twofold. First, we demonstrate the employment of ChatGPT to understand and annotate the content published in software repositories. Second, we provide evidence of hidden risk in educational repositories contributing to the opportunities of potential threats and malicious intents. We carry out a systematic study on a collection of 35.2K GitHub repositories claimed to be created for educational purposes only. First, our study finds an increasing trend in the number of such repositories published every year. Second, 9294 of them are labeled by ChatGPT as malicious, and further categorization of the malicious ones detects 14 different malware families including DDoS, keylogger, ransomware and so on. Overall, this exploratory study flags a wake-up call for the community for better understanding and analysis of software platforms.

==> 070conclusion.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AUTHOR: Christos Faloutsos
% INSTITUTION: CMU
% DATE: April 2019
% GOAL: to streamline the paper presentations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We present \method, an approach to represent a repository in an embedding vector utilizing data from three types of information sources: (a) metadata, (b) repository structure, and (c) source code available in a repository. The main idea is to aggregate the embedding representations from these three types of information. 

%The advantages of the method are 
Our work can be summarized in the following points:
\ben
\item {\bf A highly effective embedding:} \method is a comprehensive embedding approach, 
which enables us to determine similar repositories with 93\% precision.
\item {\bf Improving the state of the art:} Our approach
 outperforms the best known method, CrossSim, by a margin of  15\% in terms of precision.  Also, it  finds nearly  twice  as  many  Strongly  Similar  repositories  and  30\%  less False Positives.
\item {\bf Facilitating the identification of malware}: Our approach can classify the malware and benign repositories with 98\% precision outperforming previous studies.
\item {\bf Enabling meaningful clustering}: Our approach identifies a tree hierarchy of repositories that aligns well with their purpose and lineage.
\een
% \miii{If you want to focus on "advantages", you need to separate advantages/novelty of the method and applications}

In the future, 
we first plan to extend the work with a larger dataset and a more extensive ground truth dataset.
In fact, we would like to help develop a community-wide benchmark that will facilitate further research.
Second, we would like to extend our work to other programming languages, which hinges mostly on developing a code2vec capability for other languages.
It would be interesting to see if different languages lend themselves to embedding representations the same way we are able to do here with Java.

%Finally, we intend to open-source our code and datasets to maximize the impact of our work and facilitate follow up research.


==> 080listOfToDo.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AUTHOR: Christos Faloutsos
% INSTITUTION: CMU
% DATE: April 2019
% GOAL: to streamline the paper presentations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \todototoc
% \listoftodos

% definition of malicious repositories
% definition of malicious - part of the context in

% Many repositories are self-identified as educational, but no one has checked 
% Educational shoould be defined earlier
% There are pub repositories. some of them are self determinde to be educational,and some of them are said too be malware.
% We want to identify to public repos 
% are they enabling the spread of malware? done

% Are malicious repositories hiding under the educational label? done

% malware = malicious

% clearly malicious/incidental
% We will still consider them as malicioous/malware

% Figure 3 as the crown jewel - done
% Roughly malicious educational repos are 30% 

% Terminology maledu - malicious educational - done
% Example in page 2 - done

% We propose the systematic study to analyze

% The bigger box to contain yellow boxes - done
% Categorize shoould be renamed - done

% Classifiy the malware/Detemine the maliciousness - done

% Collect Edcuatinoal repositories
% Determine/establish maliciousness
% Determine/Categorize Malware Family

% we can get rid of workflow figure

% Workflow done
% Determining the malware
% Determining the malware family

% Labels: malware/benign/gray-area

% We found XX repos, then XX% oof them are malicious done

%%%% validation
% validation
    % both benign, 

    % To increase of our conofidence, our manual investigation corroborated 

% Methodology: A, B, C Three steps

%%%% Contribution
% percentage oof them are malicious and the number
% We also found the most dominant 
% The large content, 


% remove malware collection - done

==> makefile <==
####################################
# Author: Christos Faloutsos
# Date: March 2018
####################################

MAIN= paper
FINAL= final
SAVE-DIR=SAVE
TEXPARTS= \
    000abstract.tex \
    010introduction.tex \
    020background.tex \
    030method.tex \
    040experiment.tex \
    060conclusion.tex \
    070appendix.tex \
    080listOfToDo.tex \
    dfn.tex

BIBPARTS= BIB/*.bib BIB/catbib.bash
FIGPARTS= FIG/*.png FIG-TIKZ/*.tex
STYPARTS= sig-alternate.cls
OTHER= mkfinal.pl makefile README.txt
ALL= $(MAIN).tex $(TEXPARTS) $(BIBPARTS) $(FIGPARTS) $(STYPARTS) $(OTHER)

$(MAIN).pdf: $(MAIN).tex $(TEXPARTS) 
	pdflatex $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex

final: $(FINAL).pdf

$(FINAL).pdf: $(MAIN).tex mkfinal.pl
	perl mkfinal.pl $(MAIN).tex > $(FINAL).tex
	pdflatex $(FINAL).tex
	bibtex $(FINAL)
	pdflatex $(FINAL).tex
	pdflatex $(FINAL).tex

try: $(MAIN).tex
	pdflatex $(MAIN)


clean:
	\rm -f *.dvi $(MAIN).ps *.bbl *.aux *.log *.blg *.toc all.tar* uu \
	*~ *.bak *.lbl *.brf $(MAIN).synctex.gz \
	*.out *.soc *.tdo

spotless: clean
	\rm -f $(MAIN).ps $(MAIN).pdf
	\rm -f $(FINAL).*
	\rm -rf TST

all.tar:
	tar cvfh all.tar $(ALL)

save: all.tar
	mv all.tar $(SAVE-DIR)

